Belief-based Generation of Argumentative Claims

When engaging in argumentative discourse, skilled human debaters tailor claims to the beliefs of the audience, to construct effective arguments. Recently, the field of computational argumentation witnessed extensive effort to address the automatic generation of arguments. However, existing approaches do not perform any audience-specific adaptation. In this work, we aim to bridge this gap by studying the task of belief-based claim generation: Given a controversial topic and a set of beliefs, generate an argumentative claim tailored to the beliefs. To tackle this task, we model the people's prior beliefs through their stances on controversial topics and extend state-of-the-art text generation models to generate claims conditioned on the beliefs. Our automatic evaluation confirms the ability of our approach to adapt claims to a set of given beliefs. In a manual study, we additionally evaluate the generated claims in terms of informativeness and their likelihood to be uttered by someone with a respective belief. Our results reveal the limitations of modeling users' beliefs based on their stances, but demonstrate the potential of encoding beliefs into argumentative texts, laying the ground for future exploration of audience reach.

==> eacl21-belief-based-claim-generation-automatic-eval.tex <==
\begin{table}[t!]%
\centering%
\small
%\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{2.75pt}%
\begin{tabular}{lrrrrr}
\toprule
Approach & BLEU-1 & BLEU-3 & METEOR\\
\midrule
S2S-baseline  & 18.2\%     &     0.44\% &  \bf 16\%\\
S2S-model     & \bf \textsuperscript{*}18.4\%  & \textsuperscript{*}0.46\%  &  \bf 16\%\\
LM-baseline   & \phantom{0}9.6\%      &   0.26\%  & \phantom{0}8\% \\
LM-model    & \textsuperscript{*}12.0\%  &  0.16\%  & \textsuperscript{*}11\%\\
\bottomrule
\end{tabular}%
\caption{Scores compared to the ground-truth claims. Values marked with * are significantly better than corresponding baseline at $p$ < 0.05 (Student's $t$-test).}
\label{table-automatic-evaluation-1}%
\end{table}


%%%% OLD

\begin{table}[t!]%
%\centering%
%\renewcommand{\arraystretch}{1}
%\setlength{\tabcolsep}{2.75pt}%
%\begin{tabular}{lrrrrr}
%\toprule
%Approach & BLEU-1 & BLEU-3 & METEOR\\
%\midrule
%\textit{S2S-baseline}  & 18.25\%     &     0.44\% &  \bf 16\%\\
%\textit{S2S-model}     & \bf 18.39\%\textsuperscript{*}\hspace*{-1.5ex}  & 0.46\%\textsuperscript{*}\hspace*{-1.5ex}  &  \bf 16\%\\
%\textit{LM-baseline}   & \phantom{0}9.6\%      &   0.26\%  & \phantom{0}8\% \\
%\textit{LM-model}      & 12\%\textsuperscript{*}\hspace*{-1.5ex}  &  0.16\%  & 11\%\textsuperscript{*}\hspace*{-1.5ex}\\
%\bottomrule
%\end{tabular}%
%\caption{BLEU and METEOR scores compared to the ground-truth claims. Values marked with * are significantly better than corresponding baseline at p < 0.05 (student t-test).}
%\label{table-automatic-evaluation-1}%
\end{table}








%%%%%

==> eacl21-belief-based-claim-generation-bow-collection-eval.tex <==
\begin{table}[t!]%
\centering%
\small
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{3pt}%
\begin{tabular}{lrrrrr}
\toprule
& Cat-1 & Cat-2 & Cat-3 & Cat-4 & Cat-5\\
\midrule
Pro & 14\% & 10\% & 36\% & 34\% & 6\% \\
Con & 36\%& 2\% & 34\% & 26\% & 2\% \\
\bottomrule
\end{tabular}%
\caption{Distribution of words across categories for pro/con bag-of-words averaged across the evaluated 10 \textit{big-issues}}
\label{table-bow-collection-evaluation-1}%
\end{table}



%\begin{table*}[t!]%
%\centering%
%\renewcommand{\arraystretch}{1}
%\small
%\setlength{\tabcolsep}{3pt}%
%\begin{tabular}{lllllllllllllllllllll}
%\toprule
% & \multicolumn{2}{c}{Abortion} & \multicolumn{2}{c}{DP} & \multicolumn{2}{c}{GM} & \multicolumn{2}{c}{DL} & \multicolumn{2}{c}{GW} & \multicolumn{2}{c}{EP} & \multicolumn{2}{c}{MM} & \multicolumn{2}{c}{SB} & \multicolumn{2}{c}{MW} & \multicolumn{2}{c}{BF} \\
%\midrule
% & pro & con & pro & con & pro & con & pro & con & pro & con & pro & con & pro & con & pro & con & pro & con & pro & con \\
%\midrule
%score (5) & 24\%& 4\%& 4\%& 0\%& 12\%& 12\%& 8\%& 4\%& 0\%& 0\%& 0\%& 0\%& 4\%& 0\%& 16\%& 0\%& 0\%& 0\%& 0\%& 0\% \\ 
%score (4) & 12\%& 32\%& 4\%& 24\%& 36\%& 24\%& 40\%& 28\%& 60\%& 12\%& 36\%& 32\%& 60\%& 44\%& 32\%& 28\%& 12\%& 8\%& 48\%& 20\%\\
%score (3) \\
%score (2) \\
%score (1) \\
%\bottomrule
%\end{tabular}%
%\caption{}
%\label{table-bow-collection-evaluation}%
%\end{table*}


==> eacl21-belief-based-claim-generation-bow-collection-example.tex <==
\begin{table}[h!]%
	\centering%
	\small
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{4pt}%
	\begin{tabular}{lp{1cm}p{1cm}p{1cm}p{1cm}}
		\toprule
		& \bf Irrelevant & \multicolumn{3}{c}{\bf Relevant}\\
		\cmidrule(l@{0pt}r@{0pt}){2-2}\cmidrule(l@{5pt}r@{0pt}){3-5}
		Words & \bf c1 & \bf c2 & \bf c3 & \bf c4\&c5\\
		\midrule
		Pro & goes, homemade & murder, alive, illegal & aborted, procedures  & option, fetus, mother, right\\
		\midrule
		Con & getting, doubles & -- & delivery, rate, abort & contraception, conception, sanctity\\
		\bottomrule
	\end{tabular}%
	\caption{Example Pro/Con words for each category for \textit{Abortion} as a big issues}
	\label{table-bow-examples}%
\end{table}

==> eacl21-belief-based-claim-generation-manual-eval-2.tex <==
\begin{table}[t!]%
\centering%
\small
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{3pt}%
\begin{tabular}{lrrrr}
\toprule
Approach & All & Lv. 4 & Lv.3 & Lv. 2\\
\midrule
LM-baseline	   & 1.8     & \bf 2.5& 1.9     & 1.4 \\
LM-model		   & \bf 2.1 &  2.3   & \bf 2.5 & \bf 1.5  \\
LM-model (manual) & 2.0     &  2.3   & 2.2     & 1.5 \\
\midrule
Ground Truth			   & 2.0     &  1.9    & 1.8     & 2.2\\
\bottomrule
\end{tabular}%
\caption{Manual Evaluation: Average score reflecting claim informativeness regarding the topic (higher is better). Results are shown overall sample (All), and for each topic and \textit{big-issue} relation level.}
\label{table-manual-evaluation-2}%
\end{table}

==> eacl21-belief-based-claim-generation-manual-eval.tex <==
\begin{table*}[t!]%
\centering%
\small
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{3pt}%
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
Approach & \multicolumn{3}{c}{ALL} & \multicolumn{3}{c}{Relation Level-4} & \multicolumn{3}{c}{Relation Level-3} & \multicolumn{3}{c}{Relation Level-2}\\
\cmidrule(l@{\tabcolsep}r@{\tabcolsep}){2-4}\cmidrule(l@{\tabcolsep}r@{\tabcolsep}){5-7}\cmidrule(l@{\tabcolsep}r@{\tabcolsep}){8-10}\cmidrule(l@{\tabcolsep}r@{\tabcolsep}){11-13}
						   & HIT & MISS & UNK & HIT & MISS & UNK & HIT & MISS & UNK & HIT & MISS & UNK\\
\midrule
LM-baseline	   & 44\% & 34\% & \bf 22\% &  50\% & 50\% & \bf 0\% &   55\% & 31\% & 14\% &  \bf 27\% & 20\% & \bf 53\% \\
LM-model		   & 37\% & 32\% & 31\% &  35\% & 38\% & 27\% &  59\% & 41\% & \bf 0\% &   13\% & \bf 13\% & 74\% \\
LM-model (manual) & \bf 45\% & \bf 26\% & 28\% & \bf 50\% & \bf 31\% & 19\% &  \bf 61\% & \bf 28\% & 11\% &  25\% & 18\% & 56\% \\
\midrule
Ground Truth			   & 42\% & 30\% & 28\% &  38\% & 42\% & 19\% &  64\% & 27\% & 9\% &   27\% & 19\% & 54\% \\
\bottomrule
\end{tabular}%
\caption{Manual Evaluation: Percentage of cases where the majority of the annotators correctly (HIT), incorrectly (MISS) predicted the stance on the corresponding \textit{big-issue}, or couldn't predict the stance (UNK) form the generated claim. Results are shown overall the sample (ALL), and for each topic/\textit{big-issue} relation level.}
\label{table-manual-evaluation}%
\end{table*}

%\begin{table}[t!]%
%	\centering%
%	\renewcommand{\arraystretch}{1}
%	\setlength{\tabcolsep}{3pt}%
%	\begin{tabular}{lllll}
%		\toprule
%		Approach & ALL & LVL-4 & LVL-3 & LVL-2\\
%		\midrule
%		\textit{LM-baseline}	   &    44\% & \bf 50\% &     55\% & \bf 27\%\\
%		\textit{LM-model}		   &    37\% &     35\% &     59\% & 13\%\\
%		\textit{LM-model (manual)} &\bf 45\% & \bf 50\% & \bf 61\% & 25\%\\
%		\midrule
%		Ground Truth			   & 42\%    &     39\% & 64\% & 27\%\\
%		\bottomrule
%	\end{tabular}%
%	\caption{Manual Evaluation}
%	\label{table-manual-evaluation}%
%\end{table}


%\begin{table}[t!]%
%\centering%
%\renewcommand{\arraystretch}{1}
%\setlength{\tabcolsep}{3pt}%
%\begin{tabular}{lllll}
%\toprule
%Approach & ALL & LVL-4 & LVL-3 & LVL-2\\
%\midrule
%\textit{LM-baseline}	   &    57\% &     50\% &     64\% & 57\%\\
%\textit{LM-model}		   &    54\% &     47\% &     59\% & 50\%\\
%\textit{LM-model (manual)} &\bf 64\% & \bf 62\% & \bf 68\% & \bf 58\%\\
%\midrule
%Ground Truth			   & 58\%    &     48\% & 70\% & 58\%\\
%\bottomrule
%\end{tabular}%
%\caption{Manual Evaluation: percentage of cases where the majority of the annotators were able to predict the correct stance on the \textit{big-issue} form the generated claim.}
%\label{table-manual-evaluation}%
%\end{table}
